Multi-Agent Common Knowledge Reinforcement Learning

Cooperative multi-agent reinforcement learning often requires decentralised policies, which severely limit the agents' ability to coordinate their behaviour. In this paper, we show that common knowledge between agents allows for complex decentralised coordination. Common knowledge arises naturally in a large number of decentralised cooperative multi-agent tasks, for example, when agents can reconstruct parts of each others' observations. Since agents an independently agree on their common knowledge, they can execute complex coordinated policies that condition on this knowledge in a fully decentralised fashion. We propose multi-agent common knowledge reinforcement learning (MACKRL), a novel stochastic actor-critic algorithm that learns a hierarchical policy tree. Higher levels in the hierarchy coordinate groups of agents by conditioning on their common knowledge, or delegate to lower levels with smaller subgroups but potentially richer common knowledge. The entire policy tree can be executed in a fully decentralised fashion. As the lowest policy tree level consists of independent policies for each agent, MACKRL reduces to independently learnt decentralised policies as a special case. We demonstrate that our method can exploit common knowledge for superior performance on complex decentralised coordination tasks, including a stochastic matrix game and challenging problems in StarCraft II unit micromanagement.

==> core/0_abstract.tex <==
\begin{abstract}
Cooperative multi-agent reinforcement learning often requires decentralised policies, or 
uses them to cope with action spaces that grow exponentially in the number 
of agents. However, such policies severely limit the agents' ability 
to coordinate their behaviour.
In this paper, we show that the use of common knowledge allows for complex decentralised coordination without the need for temporally extended communication protocols.
Common knowledge arises naturally in a large number of decentralised cooperative multi-agent tasks, for example when all agents can reliably observe entities in their own field of view 
and know the fields of view of other agents. 
The quantity and quality of common knowledge available generally varies across agent groups, where larger groups tend to share less common knowledge than smaller subgroups. Hence, algorithms exploiting common knowledge need to be able to automatically select the right level of coordination. In this paper, we propose \emph{multi-agent common knowledge reinforcement learning} (\method), a novel stochastic actor-critic algorithm that allows to learn complex coordination based on common knowledge by using a fully decentralisable hierarchical policy substructure that strikes a middle ground between joint and independent learning. We demonstrate that \method~ can exploit common knowledge for superior performance on complex decentralised coordination tasks, including a stochastic matrix game and challenging coordination problems in StarCraftII unit micromanagement.






\end{abstract}



==> core/5_pairwise.tex <==
\section{Multi-Agent Common Knowledge Reinforcement Learning}
\label{sec:method}

\sw{What happened to explicitly pointing out that MACKRL is a generalisation of IL?}
 
The key idea behind \method~is to learn decentralised policies that are nonetheless coordinated.  
\method~learns centralised policies that can be executed in a decentralised fashion 
by conditioning the joint policy  $\pi^\g(\vu_{\text{env}}^\g |\mathcal{I}^\g(\tau^a))$ 
over joint action space $\mathcal{U}_{\text{env}}^\g $ of a group of agents $\g$
only on the group's trajectory of common knowledge,   
$\tau^\g=\mathcal{I}^\g(\tau^a)$.
Since all agents $a \in \g$ can deduce $\tau^\g$ with $\mathcal{I}^\g(\tau^a)$ 
and the shared random seed, \sw{make the random seed an explicit variable and input to the function} 
they can  sample the same joint action $\vu_{\text{env}}^\g$ 
and execute their individual component $u_\text{env}^a$.%

If $\mathcal{I}^\g(\tau^a)$ is sufficiently informative, then in principle it 
is possible to learn a $\pi^\g$ that chooses high quality joint actions. 
Otherwise, it may be 
preferable for $\g$ to delegate action selection to smaller subgroups.  
Coordination would no longer occur across the subgroups, but action selection 
within each subgroup could condition on a richer common knowledge signal.  
Furthermore, the choice between acting and delegating must itself be 
decentralisable amongst the agents in $\g$ and can thus only condition on 
$\mathcal{I}^\g(\tau^a)$.



\method, illustrated in Figure~\ref{fig:mackrl}, tackles this problem using a three-level hierarchy of controllers.  At the top level, the controller $\pips$ is a \emph{pair selector} that is not allowed to directly select a joint action but can only choose among pairwise partitions, i.e., it must group the agents into non-overlapping pairs.  If there are an odd number of agents, then one agent is put in a singleton group.  At the second level, each controller $\pipc$ is a \emph{pair controller} whose action space consists of the joint action space of the pair of agents plus a delegate action $u_d$ that further partitions the pair into singletons: %
  $\mathcal{U}_\g = \mathcal{U}^a_\text{env} \times \mathcal{U}^{a'}_\text{env} \union \{u_d\}$, %
 where $\g = \{a,a'\}$.  At the third level, each controller selects an individual action $u^a_\text{env}$ for a single agent $a$. %

\begin{figure}[t]
    \vspace{-0.8em}
    \begin{center}
\includegraphics[width=0.95\textwidth]{figures/mackrl}
    \end{center}
    \vspace{-0.5em}
 	\caption{Pairwise MACKRL. Left: the pair selector must assign agents to pairs (plus a singleton in this case). Middle: the pair controller can either partition the pair or select among the pair's joint actions; Right, at the last level, the controller must select an action for a single agent.}
    \label{fig:mackrl}
    \vspace{-1.0em}
\end{figure}

Algorithm \ref{alg:mackrl} \sw{something is wrong with the numbering here} summarises \method's hierarchical action selection. Since the hierarchical controllers condition only on the common knowledge
$\mathcal{I}^\g(\tau^a)$, 
which is the same for each agent $a \in \Set G$,
the selected joint actions can be executed 
in a decentralised fashion without direct communication.

\begin{algorithm}[b!]
\begin{algorithmic}
\Function{getAction}{$\tau^a_{t}$}
\State Set $\vu_{\text{env}} = \mathbf{0}$  \Comment{Initialize joint action}
\State Set $\text{b} = \left[\mathcal{A} \right] $  \Comment{Initialize group buffer}
\While{\textbf{not} b.empty()}  
\State Set $\g= \text{b.pop()}$ \Comment{Get the next group from buffer}
\State Sample $u^\g \sim \pi^\g(u^\g |\mathcal{I}^\g(\tau^a_t)) $ 
  \If{ $u^\g  \in   \mathcal{U}^\text{env}_\g $}  \Comment{Sample a joint action for $\g$} 
\State $\vu_\text{env}[\g] = u^\g $ \Comment{Assign joint action elements} 
\Else \Comment{Delegate to selected partitions}
\For{$\g' \in u^\g $}	
\State $\text{b.push}(\g')$ \Comment{Add $\g'$ in partition $u^\g$} 
\EndFor
  \EndIf
  \EndWhile
\Return $\vu_{\text{env}}$
\EndFunction
\end{algorithmic}
\caption{Action Selection in MACKRL \sw{dependence on shared random seed should be explicit here too.}} \label{alg:mackrl}
\end{algorithm}





However, rather than training a set of factorised policies, 
one for each agent, 
we train the marginalised joint policy $p(\vu_{\text{env}}|s)$
induced by the hierarchical sampling process:
\begin{equation}
	p(\vu_{\text{env}}|s) = \sum_{\text{path} \in \text{Paths}} 
	p(\vu_{\text{env}}|s, \text{path}) p(\text{path} |s),
\end{equation}
where $\text{Paths}$ is the set of all possible action assignments 
of the three levels of hierarchical controllers, i.e.,
each path corresponds to a specific action choice of the pair-selector, pair-controller, and individual policies.
The left diagram in Figure~\ref{fig:mackrl} \sw{I don't see solid or dashed lines in the figure.} shows this process: only one path 
(solid lines) is sampled for action selection.
However, all other paths (dotted lines) are considered in order to calculate 
the joint policy. With more than three agents, a particular group $\g$ may 
appear in multiple paths, in which case its policy may be cached to save 
computation. Controllers may also share parameters, enabling batching across 
different groups.

In general, sampling from a joint probability is problematic 
since the joint action space grows exponentially in the number of agents. 
Furthermore, evaluating the joint probability 
requires central state information, and thus cannot be decentralised.
The key insight of \method~is that we can use the hierarchical, 
decentralised process of Algorithm \ref{alg:mackrl} for sampling actions, 
while the marginal probabilities need to be computed 
only during centralised training in order to obtain the joint probability 
of the selected joint action.

To train these policies, we use Central-V, a multi-agent actor-critic algorithm 
with a centralised critic \citep{foerster2017counterfactual}. \sw{Could we use other algorithms instead?}
Unlike the decentralised policy, 
we condition the critic on the central state 
and the last actions of all agents.
We do not use the counterfactual baseline also proposed by \citet{foerster2017counterfactual} because \method, by inducing
 a correlated  probability across the joint action space, effectively turns training into a single agent problem and hence renders the baseline inapplicable.

The gradient with respect to the policy parameters $\theta$ is:
\begin{equation}
	\nabla_{\theta} J^p_t = A_t \;  
	\nabla_{\theta}  \log(p(\vu_{\text{env}, t}|s_t) ),
\end{equation}
where $A_t = (r_{t+1} + \gamma V(s_{t+1}, \vu_{\text{env},t}) 
-  V(s_{t}, \vu_{\text{env},t-1} ))$ 
is an estimate of the advantage.
The value function is learned by gradient descent 
on the TD($\lambda$) loss
\citep{sutton1998reinforcement}. %
As in Central-V, the critic is trained on-policy 
using samples from the environment, 
and all controllers within one layer of the hierarchy share parameters. 

In our experiments, all policies are implemented as recurrent neural networks, while the critics are feed-forward and use full state information. Table \ref{tab:pairwise} \sw{in the Supplementary Material} describes the inputs and action spaces at each level of the hierarchy. Parameters are shared across controllers within each of the second and third levels of the hierarchy.  Therefore, we also feed in the agent index or index pairs into the policy. 










Because \method~trains a joint policy in a centralised fashion, it is 
an actor-critic algorithm with a particular form of policy for the 
actor. Consequently, the standard convergence results for actor-critic methods 
\citep{konda1999actor}, which do not depend on the policy parameterisation (but 
do require a number of other assumptions), also hold for our algorithm. \sw{doesn't compatibility depend on the policy parameterisation?}




By considering only pairwise partitions, \method~avoids the otherwise large joint action spaces for 
controllers of 
large groups of agents. Nonetheless, the number of possible pair partitions grows 
rapidly with the number of agents (e.g. when $n=11$, there are $10395$ 
partitions of agents into pairs). A simple way to 
overcome this combinatorial explosion is to restrict 
the set of considered agent partitions, by, e.g., choosing a random fixed 
subset 
at the beginning of training. More sophisticated pruning mechanisms could use 
domain knowledge or learning to restrict the policies to relevant partitions. 
In Section \ref{sec:results}, we demonstrate experimentally that,
for remarkably small subsets of partitions, evaluating random subsets performs 
comparably to evaluating all partitions.

In the Supplementary Material, we also consider a generalisation of \method~to arbitrary partitions and hierarchies, though in such cases both the number of possible partitions and groups per partition can be large, likely making learning difficult.




==> core/convergence.tex <==
\section{Convergence proofs}
\newcommand{\smallfrac}[2]{ {\textstyle \frac{#1}{#2}} }
\newcommand{\grad}{\nabla\!}

\begin{mythm}
	For Boltzmann \method~policies $\pi^\g$, 
	with linear utility functions,
	exists a compatible Q-value function 
	in the sense of Theorem 2 in \citet{sutton1999policy}.
\end{mythm}

\begin{proof}
We assume that each $\pi^\g$ in \method~is a Boltzmann distribution 
with linear utility function $f^\g$,
which have basis functions $\phi^\g$ and parameters $\ve\theta_\g \in \R^m$:
\begin{equation}
	\pi^\g\!(\vu^\g|\tau^\g) := 
	\smallfrac{\exp(f^\g\!(\vu^\g|\tau^\g))}
	{\sum_{\vu'^\g \in \Set U^\g} \exp(f^\g\!(\vu'^\g|\tau^\g))} \,,
	\qquad \text{with} \qquad
	f^\g\!(\vu^\g|\tau^\g) := \ve\theta^\top_\g \ve\phi^\g\!(\vu^\g|\tau^\g) \,.
\end{equation}
Recall that the common history $\tau^\g$ of a group $\g$ can 
be derived from the history of each member,
i.e., $\tau^\g := \Set I^\g(\tau^a, \xi), \forall a \in \g$.
The gradient of this policy $\pi^\g$ 
w.r.t.~the joint policy parameters $\ve \theta$,
which include $\ve\theta_\g$, is:
\begin{equation} \label{eq:grad_group}
	\grad_{\theta} \pi^\g\!(\vu^\g|\tau^\g_t)
	\quad = \quad \delta_{\theta\theta_\g} \;
		\pi^\g\!(\vu^\g|\tau^\g_t) \Big(
			\ve\phi^\g\!(\vu^\g|\tau^\g)t)
			- \!\!\!\!{\textstyle \sum\limits_{
						\vu'^\g \in \Set U^\g_\env}}\!\!\!\!
				\pi^\g\!(\vu'^\g|\tau^\g_t) \,
				\ve\phi^\g\!(\vu'^\g|\tau^\g_t)
		\Big) \,,
\end{equation}
where $\delta_{\theta\theta_\g}$ denotes the Kronecker delta,
which is 1 for the gradient w.r.t.~$\theta_\g$ and 0 otherwise.

For a compatible linear Q-value function $q_{\psi}$
in the sense of Theorem 2 in \citet{sutton1999policy},
which is parameterised with $\ve\psi \in \R^m$
and conditions on joint actions $\vu_\env \in \Set U_\env$,
histories $\ve\tau_t := \{\tau_t^a\}_{a \in \Set A}$ 
and prior knowledge $\xi$, holds:
\begin{equation}
	\grad_{\psi} q_\psi(\ve\tau_t, \xi, \vu_\env)
	\quad=\quad \frac{\grad_{\theta} \pi(\vu_\env|\ve\tau_t, \xi)}%
				{\pi(\vu_\env|\ve\tau_t, \xi)} \,.
\end{equation}
We will now inductively construct a compatible set 
of basis functions for $q_\psi$ for a given \method~policy.
First we define the {\em marginalised policy} $\bar\pi^\g$,
which evaluates Algorithm \ref{alg:central} for sub-policy $\pi^\g$:
\begin{equation}
	\bar\pi^\g(\vu^\g_\env|\ve\tau_t, \xi) 
	\quad:=\quad 
		\pi^\g(\vu^\g_\env|\tau^\g_t) +
		\sum_{\vu^\g \not\in\, \Set U^\g_\env} \pi^\g(\vu^\g |\tau^\g_t)
			\prod_{\g' \in \vu^\g} \bar\pi^{\g'}(\vu^{\g'}|\ve\tau_t, \xi) \,.
\end{equation}
In the leaf-case of the \method~policy tree, 
only environmental actions of the group in questions can be selected,
that is, $\bar\pi^\g(\vu^\g_\env|\ve\tau_t, \xi) 
= \pi^\g(\vu^\g_\env|\tau^\g_t)$,
and the gradient is given in \eqref{eq:grad_group}.
The gradient over a non-leaf marginal policy $\bar\pi^\g$ is:
\begin{eqnarray} \label{eq:grad_marginal}
	\grad_{\theta} \bar\pi^\g\!(\vu^\g_\env|\ve\tau_t, \xi) 
	&=& \grad_{\theta} \pi^\g\!(\vu^\g_\env|\tau^\g_t) \;\;+
		{\textstyle\sum\limits_{\vu^\g \not\in\, \Set U^\g_\env}}
			\grad_{\theta} \pi^\g\!(\vu^\g |\tau^\g_t)
			{\textstyle\prod\limits_{\g' \in \vu^\g}}  
				\bar\pi^{\g'}\!\!(\vu^{\g'}|\ve\tau_t, \xi) 
\\ \nonumber
	&& + {\textstyle\sum\limits_{\vu^\g \not\in\, \Set U^\g_\env}}
			\pi^\g\!(\vu^\g |\tau^\g_t) 
			{\textstyle\sum\limits_{\g' \in \vu^\g}}
				\grad_{\theta}\bar\pi^{\g'}\!\!(\vu^{\g'}|\tau_t^\g)
				\hspace{-4mm}{\textstyle\prod\limits_{\g" \in \vu^\g \setminus \{\g'\}}} 
					\hspace{-4mm}\bar\pi^{\g"}\!\!(\vu^{\g"}|\ve\tau_t, \xi) \,.
\end{eqnarray}
It follows by induction that the gradient of the root policy
$\grad_\theta \bar\pi^{\Set A} = \grad_\theta \pi$
can be computed by recursion of \eqref{eq:grad_marginal} through the tree.
Furthermore, the part of the gradient 
that corresponds to parameters $\ve\theta_\g$ is
a linear combination of the sub-policies' basis functions $\ve\phi^\g$.
Using the basis functions $\ve\phi^q := \grad_\theta \bar\pi^{\Set A} 
/ \bar\pi^{\Set A}$ for $q_\psi$ 
yields therefore a compatible Q-value function to any \method~policy.
\end{proof}

\begin{mythm}
	For any differentiable \method~policy 
	exists a compatible linear Q-value function 
	in the sense of Theorem 2 of \citet{sutton1999policy}.
\end{mythm}
\begin{proof}
	A compatible Q-value function $q_{\psi}$,
	which is parameterised with $\ve\psi \in \R^m$
	and conditions on joint actions $\vu_\env \in \Set U_\env$,
	histories $\ve\tau_t := \{\tau_t^a\}_{a \in \Set A}$ 
	and prior knowledge $\xi$, 
	is compatible in the sense of Theorem 2 in \citet{sutton1999policy} 
	if the following condition holds:
	\begin{equation}
		\grad_{\psi} q_\psi(\ve\tau_t, \xi, \vu_\env)
		\quad=\quad \frac{\grad_{\theta} \pi(\vu_\env|\ve\tau_t, \xi)}%
					{\pi(\vu_\env|\ve\tau_t, \xi)} \,,
		\qquad \forall \vu_\env, \forall\ve\tau_t, \forall\xi \,.
	\end{equation}
	For each differentiable \method~policy $\pi$,
	one can therefore use the right hand side of 
	this equation to construct the bases $\ve \phi$
	for a linear Q-value function $q_\psi(\ve\tau_t, \xi, \vu_\env)
	= \ve\psi^\top \ve\phi(\ve\tau_t, \xi, \vu_\env)$.
\end{proof}

